Hybrid Neural Representations for Spherical Data

In this paper, we study hybrid neural representations for spherical data, a domain of increasing relevance in scientific research. In particular, our work focuses on weather and climate data as well as comic microwave background (CMB) data. Although previous studies have delved into coordinate-based neural representations for spherical signals, they often fail to capture the intricate details of highly nonlinear signals. To address this limitation, we introduce a novel approach named Hybrid Neural Representations for Spherical data (HNeR-S). Our main idea is to use spherical feature-grids to obtain positional features which are combined with a multilayer perception to predict the target signal. We consider feature-grids with equirectangular and hierarchical equal area isolatitude pixelization structures that align with weather data and CMB data, respectively. We extensively verify the effectiveness of our HNeR-S for regression, super-resolution, temporal interpolation, and compression tasks.

==> appdx/task_details.tex <==
\section{Task Details}
\textbf{Super-resolution.} The study applies two settings for enhancing the resolution of CMB, weather, and climate data: $\times2$ and $\times4$. In the $\times2$ setting, the model is trained using $361 \times 720$ training points, each representing a 0.50$^\circ$ degree. For the $\times4$ setting, training involves $181\times 360$ points, with each point representing a 1.00$^\circ$ degree. The model's performance is assessed on its ability to predict data at a finer resolution of 0.25$^\circ$, across a total of $721\times 1440$ points. In the context of CMB super-resolution, the $\times2$ setting involves training on data downsampled to $N_\text{side}=1024$, yielding approximately 10M training points at a resolution of about $N\mu$min. For the $\times4$ setting, the training data is further downsampled to $N_\text{side}=512$, with around 30K points. The prediction task targets data with $N_\text{side}=2048$, encompassing about 50M points at the full resolution provided by the Planck satellite.

\textbf{Regression.} The regression task involves dividing data points into training and testing sets in an 8:2 ratio. Specifically, for weather and climate data, the split is conducted on geopotential and temperature datasets that total $721\times 1440$ points, resulting in approximately 83K training points and 20K test points. For CMB data, the split includes 50M points, allocating 40M for training and 10M for testing.

\textbf{Temporal Interpolation.} This task employs two temporal resolutions: daily and weekly, with a total of 30 data snapshots sampled. Here, snapshots indicates the data which represents the captured moment. The spacing between snapshots corresponds to the chosen temporal resolution. Training data is constructed by selecting the first snapshot, skipping the next, and then selecting the third snapshot. Conversely, test data is compiled by skipping the first snapshot, selecting the second, and continuing this pattern. This method ensures a consistent and desired time step between training and test datasets.

\textbf{Compression.} 


==> figure/appdx_cmb_sr_2x.tex <==
\begin{table*}[h]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}[width=0.93\textwidth]{p{0.05\textwidth}cccccp{0.05\textwidth}}
    \toprule
         & Reference & RELU+P.E. & WIRE & FFN & \textbf{Ours} & \\
         \midrule
         % &  & $24.42$ dB &  $25.99$ dB & $28.39$ dB & $\mathbf{38.72}$ dB & \\
         % \midrule
         % visualization for regression
        \raisebox{-0.73\height}[0pt][0pt]{\includegraphics[height=8.6\normalbaselineskip,width=0.05\textwidth]{figure/error_bar_left.pdf}}
         & \begin{minipage}{0.15\textwidth}
             \includegraphics[width=\linewidth, height=1.9cm]{figure/cmb_reg/relu_pred.png}
         \end{minipage} &
              \begin{minipage}{0.15\textwidth}
             \includegraphics[width=\linewidth, height=1.9cm]{figure/cmb_reg/relu_pred.png}
         \end{minipage} &
         %      \begin{minipage}{0.15\textwidth}
         %     \includegraphics[width=\linewidth, height=1.9cm]{figure/cmb_reg/siren_pred.png}
         % \end{minipage} &
         %      \begin{minipage}{0.15\textwidth}
         %     \includegraphics[width=\linewidth, height=1.9cm]{figure/cmb_reg/shinr_pred.png}
         % \end{minipage} &
              \begin{minipage}{0.15\textwidth}
             \includegraphics[width=\linewidth, height=1.9cm]{figure/cmb_reg/wire_pred.png}
         \end{minipage} &
              \begin{minipage}{0.15\textwidth}
             \includegraphics[width=\linewidth, height=1.9cm]{figure/cmb_reg/gauss_pred.png}
         \end{minipage} &
              \begin{minipage}{0.15\textwidth}
             \includegraphics[width=\linewidth, height=1.9cm]{figure/cmb_reg/ours_pred.png}
         \end{minipage} &
         \raisebox{-0.725\height}[0pt][0pt]{\includegraphics[height=8.6\normalbaselineskip,width=0.05\textwidth]{figure/error_bar.png}}
         \\
         
         % errormap for regression
         %         \begin{minipage}{0.15\textwidth}
         %     \includegraphics[height=1.9cm]{figure/error_baer.pdf}
         % \end{minipage}
         % &
         & &
              \begin{minipage}{0.15\textwidth}
             \includegraphics[width=\linewidth, height=1.9cm]{figure/cmb_reg/relu_error.png}
         \end{minipage} &
         %      \begin{minipage}{0.15\textwidth}
         %     \includegraphics[width=\linewidth, height=1.9cm]{figure/cmb_reg/siren_error.png}
         % \end{minipage} &
         %      \begin{minipage}{0.15\textwidth}
         %     \includegraphics[width=\linewidth, height=1.9cm]{figure/cmb_reg/shinr_error.png}
         % \end{minipage} &
              \begin{minipage}{0.15\textwidth}
             \includegraphics[width=\linewidth, height=1.9cm]{figure/cmb_reg/wire_error.png}
         \end{minipage} &
              \begin{minipage}{0.15\textwidth}
             \includegraphics[width=\linewidth, height=1.9cm]{figure/cmb_reg/gauss_error.png}
         \end{minipage} &
              \begin{minipage}{0.15\textwidth}
             \includegraphics[width=\linewidth, height=1.9cm]{figure/cmb_reg/ours_error.png}
         \end{minipage} \\
         % & \multicolumn{3}{c}{\includegraphics[width=0.3\linewidth]{figure/error_bar.pdf}} & \\
         \bottomrule
    \end{tabular}
    }
    \captionof{figure}{\textbf{Visualizations of regression for CMB data.} The predictions (top) and error maps (bottom) of the top-4 methods are shown in our display. The unit for the visualizations are microkelvin ($\mu$K). In predicting the CMB temperature throughout the full sky region, our model surpasses other baselines.}
    \label{fig:vis_cos}
\end{table*}

==> figure/appdx_cmb_sr_4x.tex <==
\begin{table*}[h]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}[width=0.93\textwidth]{p{0.05\textwidth}cccccp{0.05\textwidth}}
    \toprule
         & Reference & RELU+P.E. & WIRE & FFN & \textbf{Ours} & \\
         \midrule
         % &  & $24.42$ dB &  $25.99$ dB & $28.39$ dB & $\mathbf{38.72}$ dB & \\
         % \midrule
         % visualization for regression
        \raisebox{-0.73\height}[0pt][0pt]{\includegraphics[height=8.6\normalbaselineskip,width=0.05\textwidth]{figure/error_bar_left.pdf}}
         & \begin{minipage}{0.15\textwidth}
             \includegraphics[width=\linewidth, height=1.9cm]{figure/cmb_reg/relu_pred.png}
         \end{minipage} &
              \begin{minipage}{0.15\textwidth}
             \includegraphics[width=\linewidth, height=1.9cm]{figure/cmb_reg/relu_pred.png}
         \end{minipage} &
         %      \begin{minipage}{0.15\textwidth}
         %     \includegraphics[width=\linewidth, height=1.9cm]{figure/cmb_reg/siren_pred.png}
         % \end{minipage} &
         %      \begin{minipage}{0.15\textwidth}
         %     \includegraphics[width=\linewidth, height=1.9cm]{figure/cmb_reg/shinr_pred.png}
         % \end{minipage} &
              \begin{minipage}{0.15\textwidth}
             \includegraphics[width=\linewidth, height=1.9cm]{figure/cmb_reg/wire_pred.png}
         \end{minipage} &
              \begin{minipage}{0.15\textwidth}
             \includegraphics[width=\linewidth, height=1.9cm]{figure/cmb_reg/gauss_pred.png}
         \end{minipage} &
              \begin{minipage}{0.15\textwidth}
             \includegraphics[width=\linewidth, height=1.9cm]{figure/cmb_reg/ours_pred.png}
         \end{minipage} &
         \raisebox{-0.725\height}[0pt][0pt]{\includegraphics[height=8.6\normalbaselineskip,width=0.05\textwidth]{figure/error_bar.png}}
         \\
         
         % errormap for regression
         %         \begin{minipage}{0.15\textwidth}
         %     \includegraphics[height=1.9cm]{figure/error_baer.pdf}
         % \end{minipage}
         % &
         & &
              \begin{minipage}{0.15\textwidth}
             \includegraphics[width=\linewidth, height=1.9cm]{figure/cmb_reg/relu_error.png}
         \end{minipage} &
         %      \begin{minipage}{0.15\textwidth}
         %     \includegraphics[width=\linewidth, height=1.9cm]{figure/cmb_reg/siren_error.png}
         % \end{minipage} &
         %      \begin{minipage}{0.15\textwidth}
         %     \includegraphics[width=\linewidth, height=1.9cm]{figure/cmb_reg/shinr_error.png}
         % \end{minipage} &
              \begin{minipage}{0.15\textwidth}
             \includegraphics[width=\linewidth, height=1.9cm]{figure/cmb_reg/wire_error.png}
         \end{minipage} &
              \begin{minipage}{0.15\textwidth}
             \includegraphics[width=\linewidth, height=1.9cm]{figure/cmb_reg/gauss_error.png}
         \end{minipage} &
              \begin{minipage}{0.15\textwidth}
             \includegraphics[width=\linewidth, height=1.9cm]{figure/cmb_reg/ours_error.png}
         \end{minipage} \\
         % & \multicolumn{3}{c}{\includegraphics[width=0.3\linewidth]{figure/error_bar.pdf}} & \\
         \bottomrule
    \end{tabular}
    }
    \captionof{figure}{\textbf{Visualizations of regression for CMB data.} The predictions (top) and error maps (bottom) of the top-4 methods are shown in our display. The unit for the visualizations are microkelvin ($\mu$K). In predicting the CMB temperature throughout the full sky region, our model surpasses other baselines.}
    \label{fig:vis_cos}
\end{table*}

==> figure/appdx_geo_reg.tex <==
\begin{table*}[h]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}[width=0.85\textwidth]{p{0.045\textwidth}cccccp{0.08\textwidth}}
    \toprule
         & Reference & RELU+P.E. & WIRE & FFN & \textbf{Ours} & \\
         \midrule
         % &  & $24.42$ dB &  $25.99$ dB & $28.39$ dB & $\mathbf{38.72}$ dB & \\
         % \midrule
         % visualization for regression
        \raisebox{-0.73\height}[0pt][0pt]{\includegraphics[height=8.6\normalbaselineskip,width=0.05\textwidth]{figure/weather_x2/temp_x2_pred_bar.png}}
         & \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_relu_pred}
         \end{minipage} &
              \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_relu_pred}
         \end{minipage} &
         %      \begin{minipage}{0.115\textwidth}
         %     \includegraphics[width=\linewidth]{figure/weather_x2/sphere_siren_pred}
         % \end{minipage} &
         %      \begin{minipage}{0.115\textwidth}
         %     \includegraphics[width=\linewidth]{figure/weather_x2/sphere_shinr_pred}
         % \end{minipage} &
              \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_wire_pred}
         \end{minipage} &
              \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_gauss_pred}
         \end{minipage} &
              \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_ours_pred}
         \end{minipage} &
         \raisebox{-0.725\height}[0pt][0pt]{\includegraphics[height=8.6\normalbaselineskip,width=0.05\textwidth]{figure/weather_x2/temp_x2_error_bar.png}}
         \\
         
         % errormap for regression
         %         \begin{minipage}{0.115\textwidth}
         %     \includegraphics[height=1.9cm]{figure/error_baer.pdf}
         % \end{minipage}
         % &
         & &
              \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_relu_error}
         \end{minipage} &
         %      \begin{minipage}{0.115\textwidth}
         %     \includegraphics[width=\linewidth]{figure/weather_x2/sphere_siren_error}
         % \end{minipage} &
         %      \begin{minipage}{0.115\textwidth}
         %     \includegraphics[width=\linewidth]{figure/weather_x2/sphere_shinr_error}
         % \end{minipage} &
              \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_wire_error}
         \end{minipage} &
              \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_gauss_error}
         \end{minipage} &
              \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_ours_error}
         \end{minipage} \\
         % & \multicolumn{3}{c}{\includegraphics[width=0.3\linewidth]{figure/error_bar.pdf}} & \\
         \bottomrule
    \end{tabular}
    }
    \captionof{figure}{\textbf{Visualizations of ($\times2$) super-resolution for temperature data.} The predictions (top) and error maps (bottom) of the top-4 methods are shown in our figure. The unit for the visualization is Kelvin ($K$). Our model outperforms other baselines in predicting the target signal across the entire domain.}
    \label{fig:vis_weather}
\end{table*}

==> figure/appdx_geo_x2.tex <==
\begin{table*}[h]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}[width=0.85\textwidth]{p{0.045\textwidth}cccccp{0.08\textwidth}}
    \toprule
         & Reference & RELU+P.E. & WIRE & FFN & \textbf{Ours} & \\
         \midrule
         % &  & $24.42$ dB &  $25.99$ dB & $28.39$ dB & $\mathbf{38.72}$ dB & \\
         % \midrule
         % visualization for regression
        \raisebox{-0.73\height}[0pt][0pt]{\includegraphics[height=8.6\normalbaselineskip,width=0.05\textwidth]{figure/weather_x2/temp_x2_pred_bar.png}}
         & \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_relu_pred}
         \end{minipage} &
              \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_relu_pred}
         \end{minipage} &
         %      \begin{minipage}{0.115\textwidth}
         %     \includegraphics[width=\linewidth]{figure/weather_x2/sphere_siren_pred}
         % \end{minipage} &
         %      \begin{minipage}{0.115\textwidth}
         %     \includegraphics[width=\linewidth]{figure/weather_x2/sphere_shinr_pred}
         % \end{minipage} &
              \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_wire_pred}
         \end{minipage} &
              \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_gauss_pred}
         \end{minipage} &
              \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_ours_pred}
         \end{minipage} &
         \raisebox{-0.725\height}[0pt][0pt]{\includegraphics[height=8.6\normalbaselineskip,width=0.05\textwidth]{figure/weather_x2/temp_x2_error_bar.png}}
         \\
         
         % errormap for regression
         %         \begin{minipage}{0.115\textwidth}
         %     \includegraphics[height=1.9cm]{figure/error_baer.pdf}
         % \end{minipage}
         % &
         & &
              \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_relu_error}
         \end{minipage} &
         %      \begin{minipage}{0.115\textwidth}
         %     \includegraphics[width=\linewidth]{figure/weather_x2/sphere_siren_error}
         % \end{minipage} &
         %      \begin{minipage}{0.115\textwidth}
         %     \includegraphics[width=\linewidth]{figure/weather_x2/sphere_shinr_error}
         % \end{minipage} &
              \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_wire_error}
         \end{minipage} &
              \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_gauss_error}
         \end{minipage} &
              \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_ours_error}
         \end{minipage} \\
         % & \multicolumn{3}{c}{\includegraphics[width=0.3\linewidth]{figure/error_bar.pdf}} & \\
         \bottomrule
    \end{tabular}
    }
    \captionof{figure}{\textbf{Visualizations of ($\times2$) super-resolution for temperature data.} The predictions (top) and error maps (bottom) of the top-4 methods are shown in our figure. The unit for the visualization is Kelvin ($K$). Our model outperforms other baselines in predicting the target signal across the entire domain.}
    \label{fig:vis_weather}
\end{table*}

==> figure/appdx_geo_x4.tex <==
\begin{table*}[h]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}[width=0.85\textwidth]{p{0.045\textwidth}cccccp{0.08\textwidth}}
    \toprule
         & Reference & RELU+P.E. & WIRE & FFN & \textbf{Ours} & \\
         \midrule
         % &  & $24.42$ dB &  $25.99$ dB & $28.39$ dB & $\mathbf{38.72}$ dB & \\
         % \midrule
         % visualization for regression
        \raisebox{-0.73\height}[0pt][0pt]{\includegraphics[height=8.6\normalbaselineskip,width=0.05\textwidth]{figure/weather_x2/temp_x2_pred_bar.png}}
         & \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_relu_pred}
         \end{minipage} &
              \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_relu_pred}
         \end{minipage} &
         %      \begin{minipage}{0.115\textwidth}
         %     \includegraphics[width=\linewidth]{figure/weather_x2/sphere_siren_pred}
         % \end{minipage} &
         %      \begin{minipage}{0.115\textwidth}
         %     \includegraphics[width=\linewidth]{figure/weather_x2/sphere_shinr_pred}
         % \end{minipage} &
              \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_wire_pred}
         \end{minipage} &
              \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_gauss_pred}
         \end{minipage} &
              \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_ours_pred}
         \end{minipage} &
         \raisebox{-0.725\height}[0pt][0pt]{\includegraphics[height=8.6\normalbaselineskip,width=0.05\textwidth]{figure/weather_x2/temp_x2_error_bar.png}}
         \\
         
         % errormap for regression
         %         \begin{minipage}{0.115\textwidth}
         %     \includegraphics[height=1.9cm]{figure/error_baer.pdf}
         % \end{minipage}
         % &
         & &
              \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_relu_error}
         \end{minipage} &
         %      \begin{minipage}{0.115\textwidth}
         %     \includegraphics[width=\linewidth]{figure/weather_x2/sphere_siren_error}
         % \end{minipage} &
         %      \begin{minipage}{0.115\textwidth}
         %     \includegraphics[width=\linewidth]{figure/weather_x2/sphere_shinr_error}
         % \end{minipage} &
              \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_wire_error}
         \end{minipage} &
              \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_gauss_error}
         \end{minipage} &
              \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_ours_error}
         \end{minipage} \\
         % & \multicolumn{3}{c}{\includegraphics[width=0.3\linewidth]{figure/error_bar.pdf}} & \\
         \bottomrule
    \end{tabular}
    }
    \captionof{figure}{\textbf{Visualizations of ($\times2$) super-resolution for temperature data.} The predictions (top) and error maps (bottom) of the top-4 methods are shown in our figure. The unit for the visualization is Kelvin ($K$). Our model outperforms other baselines in predicting the target signal across the entire domain.}
    \label{fig:vis_weather}
\end{table*}

==> figure/appdx_temp_reg.tex <==
\begin{table*}[h]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}[width=0.85\textwidth]{p{0.045\textwidth}cccccp{0.08\textwidth}}
    \toprule
         & Reference & RELU+P.E. & WIRE & FFN & \textbf{Ours} & \\
         \midrule
         % &  & $24.42$ dB &  $25.99$ dB & $28.39$ dB & $\mathbf{38.72}$ dB & \\
         % \midrule
         % visualization for regression
        \raisebox{-0.73\height}[0pt][0pt]{\includegraphics[height=8.6\normalbaselineskip,width=0.05\textwidth]{figure/weather_x2/temp_x2_pred_bar.png}}
         & \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_relu_pred}
         \end{minipage} &
              \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_relu_pred}
         \end{minipage} &
         %      \begin{minipage}{0.115\textwidth}
         %     \includegraphics[width=\linewidth]{figure/weather_x2/sphere_siren_pred}
         % \end{minipage} &
         %      \begin{minipage}{0.115\textwidth}
         %     \includegraphics[width=\linewidth]{figure/weather_x2/sphere_shinr_pred}
         % \end{minipage} &
              \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_wire_pred}
         \end{minipage} &
              \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_gauss_pred}
         \end{minipage} &
              \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_ours_pred}
         \end{minipage} &
         \raisebox{-0.725\height}[0pt][0pt]{\includegraphics[height=8.6\normalbaselineskip,width=0.05\textwidth]{figure/weather_x2/temp_x2_error_bar.png}}
         \\
         
         % errormap for regression
         %         \begin{minipage}{0.115\textwidth}
         %     \includegraphics[height=1.9cm]{figure/error_baer.pdf}
         % \end{minipage}
         % &
         & &
              \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_relu_error}
         \end{minipage} &
         %      \begin{minipage}{0.115\textwidth}
         %     \includegraphics[width=\linewidth]{figure/weather_x2/sphere_siren_error}
         % \end{minipage} &
         %      \begin{minipage}{0.115\textwidth}
         %     \includegraphics[width=\linewidth]{figure/weather_x2/sphere_shinr_error}
         % \end{minipage} &
              \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_wire_error}
         \end{minipage} &
              \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_gauss_error}
         \end{minipage} &
              \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_ours_error}
         \end{minipage} \\
         % & \multicolumn{3}{c}{\includegraphics[width=0.3\linewidth]{figure/error_bar.pdf}} & \\
         \bottomrule
    \end{tabular}
    }
    \captionof{figure}{\textbf{Visualizations of ($\times2$) super-resolution for temperature data.} The predictions (top) and error maps (bottom) of the top-4 methods are shown in our figure. The unit for the visualization is Kelvin ($K$). Our model outperforms other baselines in predicting the target signal across the entire domain.}
    \label{fig:vis_weather}
\end{table*}

==> figure/appdx_temp_x4.tex <==
\begin{table*}[h]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}[width=0.85\textwidth]{p{0.045\textwidth}cccccp{0.08\textwidth}}
    \toprule
         & Reference & RELU+P.E. & WIRE & FFN & \textbf{Ours} & \\
         \midrule
         % &  & $24.42$ dB &  $25.99$ dB & $28.39$ dB & $\mathbf{38.72}$ dB & \\
         % \midrule
         % visualization for regression
        \raisebox{-0.73\height}[0pt][0pt]{\includegraphics[height=8.6\normalbaselineskip,width=0.05\textwidth]{figure/weather_x2/temp_x2_pred_bar.png}}
         & \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_relu_pred}
         \end{minipage} &
              \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_relu_pred}
         \end{minipage} &
         %      \begin{minipage}{0.115\textwidth}
         %     \includegraphics[width=\linewidth]{figure/weather_x2/sphere_siren_pred}
         % \end{minipage} &
         %      \begin{minipage}{0.115\textwidth}
         %     \includegraphics[width=\linewidth]{figure/weather_x2/sphere_shinr_pred}
         % \end{minipage} &
              \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_wire_pred}
         \end{minipage} &
              \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_gauss_pred}
         \end{minipage} &
              \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_ours_pred}
         \end{minipage} &
         \raisebox{-0.725\height}[0pt][0pt]{\includegraphics[height=8.6\normalbaselineskip,width=0.05\textwidth]{figure/weather_x2/temp_x2_error_bar.png}}
         \\
         
         % errormap for regression
         %         \begin{minipage}{0.115\textwidth}
         %     \includegraphics[height=1.9cm]{figure/error_baer.pdf}
         % \end{minipage}
         % &
         & &
              \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_relu_error}
         \end{minipage} &
         %      \begin{minipage}{0.115\textwidth}
         %     \includegraphics[width=\linewidth]{figure/weather_x2/sphere_siren_error}
         % \end{minipage} &
         %      \begin{minipage}{0.115\textwidth}
         %     \includegraphics[width=\linewidth]{figure/weather_x2/sphere_shinr_error}
         % \end{minipage} &
              \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_wire_error}
         \end{minipage} &
              \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_gauss_error}
         \end{minipage} &
              \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_ours_error}
         \end{minipage} \\
         % & \multicolumn{3}{c}{\includegraphics[width=0.3\linewidth]{figure/error_bar.pdf}} & \\
         \bottomrule
    \end{tabular}
    }
    \captionof{figure}{\textbf{Visualizations of ($\times2$) super-resolution for temperature data.} The predictions (top) and error maps (bottom) of the top-4 methods are shown in our figure. The unit for the visualization is Kelvin ($K$). Our model outperforms other baselines in predicting the target signal across the entire domain.}
    \label{fig:vis_weather}
\end{table*}

==> figure/fig_3_errormap.tex <==

\begin{figure}[H]
    \centering
%    \includegraphics[width=0.45\textwidth, height=3cm]{case-error-map.pdf}
    \includegraphics[width=0.45\textwidth, height=3cm]{example-image-a}
    \vspace{-3mm}
    \caption{Error map by data and parameter distribution}
    \label{fig:case-error-map}
    %\vspace{-3mm}
\end{figure}
\vspace{-3mm}

==> figure/fig_3_interpolation.tex <==
\begin{figure}[t]
  \includegraphics[width=0.47\textwidth, height=5cm]{example-image-a}
   \caption{\textbf{Interpolation algorithm.} }
   \label{fig:interpolation}
\end{figure}

==> figure/fig_3_overview.tex <==
\begin{figure*}[t]
  
  % \relatedwork{Method overview}
  \includegraphics[width=\textwidth, height=5cm]{example-image-a}
  \caption{\textbf{Method overview.} }
  \label{fig:overview}
\end{figure*}

==> figure/fig_4_cli_sr.tex <==
\begin{figure}[t]
      \caption{\textbf{Visualization of super-resolution on climatology data.}  XX}
      \vspace{2mm}
      \includegraphics[width=0.47\textwidth]{figure/weather_pred.png}
      % \experiments{Prediction of Weather SR} 
      \label{fig:weather_sr_pred}
\end{figure}

==> figure/fig_4_cmb_reg.tex <==
\begin{figure}
    \centering
      \includegraphics[width=0.47\textwidth]{figure/cmb_error.png}
       \captionof{figure}{\textbf{Cosmic microwave background regression.} (TBU) }
      \label{fig:cos_cmb_reg}
\end{figure}

==> figure/fig_4_cmb_super.tex <==
\begin{figure}[t]
      \includegraphics[width=0.47\textwidth]{figure/cmb_sr_4x.pdf}
      \caption{\textbf{Cosmic microwave background super-resolution.} XX }
      \label{fig:cmb_super}
\end{figure}

==> figure/fig_4_comp.tex <==
\begin{figure}[h]      
      \includegraphics[width=0.47\textwidth]{figure/compression.pdf}
      % \vspace{0.1in}
      \caption{\textbf{The results of compression.} Circles indicate the compression methods following image compression without time encoding $t$ while $\times$s indicate video compression-like methods with time encoding $t$.}
      \label{fig:compression}
\end{figure}

==> figure/fig_4_temporal_interp.tex <==
\begin{figure*}[h]
  % \relatedwork{Method overview}
  \includegraphics[width=0.45\textwidth, height=5cm]{example-image-a}
  \caption{\textbf{Temporal interpolation (Gauss vs Ours).} }
  \label{fig:temporal}
  % \vspace{-9mm}
\end{figure*}

==> figure/fig_4_vis_weather_old.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{cccccc}
    \toprule
         Reference & RELU+P.E. & SIREN  & FFN & Ours \\
         % \midrule
         % % visualization for regression
         % \begin{minipage}{0.115\textwidth}
         %     \includegraphics[width=\linewidth]{example-image-a}
         % \end{minipage} &
         %      \begin{minipage}{0.115\textwidth}
         %     \includegraphics[width=\linewidth]{example-image-a}
         % \end{minipage} & 
         %      \begin{minipage}{0.115\textwidth}
         %     \includegraphics[width=\linewidth]{example-image-a}
         % \end{minipage} &
         %      \begin{minipage}{0.115\textwidth}
         %     \includegraphics[width=\linewidth]{example-image-a}
         % \end{minipage} &
         %      \begin{minipage}{0.115\textwidth}
         %     \includegraphics[width=\linewidth]{example-image-a}
         % \end{minipage} &
         %      \begin{minipage}{0.115\textwidth}
         %     \includegraphics[width=\linewidth]{example-image-a}
         % \end{minipage} &
         %      \begin{minipage}{0.115\textwidth}
         %     \includegraphics[width=\linewidth]{example-image-a}
         % \end{minipage} \\
         %    % errormap for regression
         %          \begin{minipage}{0.115\textwidth}
         %     \includegraphics[width=\linewidth]{example-image-a}
         % \end{minipage} &
         %      \begin{minipage}{0.115\textwidth}
         %     \includegraphics[width=\linewidth]{example-image-a}
         % \end{minipage} &
         %      \begin{minipage}{0.115\textwidth}
         %     \includegraphics[width=\linewidth]{example-image-a}
         % \end{minipage} &
         %      \begin{minipage}{0.115\textwidth}
         %     \includegraphics[width=\linewidth]{example-image-a}
         % \end{minipage} &
         %      \begin{minipage}{0.115\textwidth}
         %     \includegraphics[width=\linewidth]{example-image-a}
         % \end{minipage} &
         %      \begin{minipage}{0.115\textwidth}
         %     \includegraphics[width=\linewidth]{example-image-a}
         % \end{minipage} &
         %      \begin{minipage}{0.115\textwidth}
         %     \includegraphics[width=\linewidth]{example-image-a}
         % \end{minipage} \\
         \midrule
          % visualization for super-resolution
         \raisebox{-0.73\height}[0pt][0pt]{\includegraphics[height=8.6\normalbaselineskip,width=0.05\textwidth]{figure/weather_x2/temp_x2_pred_bar.png}}
        \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_ours_pred.png}
         \end{minipage} &
              \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_relu_pred.png}
         \end{minipage} &
              \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_siren_pred.png}
         \end{minipage} &

         %      \begin{minipage}{0.115\textwidth}
         %     \includegraphics[width=\linewidth]{figure/weather_x2/sphere_shinr_pred}
         % \end{minipage} &
         %      \begin{minipage}{0.115\textwidth}
         %     \includegraphics[width=\linewidth]{figure/weather_x2/sphere_wire_pred}
         % \end{minipage} &
              \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_gauss_pred.png}
         \end{minipage} &
              \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_ours_pred.png}
         \end{minipage} \\
                        &
              \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_relu_error.png}
         \end{minipage} &
         \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_siren_error.png}
         \end{minipage} &
         %      \begin{minipage}{0.115\textwidth}
         %     \includegraphics[width=\linewidth]{figure/weather_x2/sphere_shinr_error}
         % \end{minipage} &
         %      \begin{minipage}{0.115\textwidth}
         %     \includegraphics[width=\linewidth]{figure/weather_x2/sphere_wire_error}
         % \end{minipage} &
          \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_gauss_error.png}
         \end{minipage} &
          \begin{minipage}{0.115\textwidth}
             \includegraphics[width=\linewidth]{figure/weather_x2/sphere_ours_error.png}
         \end{minipage} &
       \raisebox{-0.725\height}[0pt][0pt]{\includegraphics[height=8.6\normalbaselineskip,width=0.05\textwidth]{figure/weather_x2/temp_x2_error_bar.png}}
        \\
         \bottomrule
    \end{tabular}
    \captionof{figure}{Visualization of prediction (above) and error map (bottom) of super-resolution for geopotential data. (TBU into more discriminative visualization).}
    \label{fig:vis_weather}
\end{table*}

==> figure/fig_cmb_reg_psnr.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figure/cmb_reg_psnr.pdf}
    \vspace{-0.1in}
    \caption{\small \textbf{Test PSNR of CMB regression.}}
    \label{fig:cmb_reg}
\end{figure}

==> figure/fig_spatial_visualization.tex <==
\begin{figure*}[t]
    \centering    

    \begin{minipage}{\textwidth}
      \caption{\textbf{Cosmic microwave background regression.} We show prediction and test curve of the cmb regression task.}
      \vspace{2mm}
      \includegraphics[width=\textwidth]{figure/cmb_error.png}
      \label{fig:cmb_reg_error}
    \end{minipage}%
    
    \begin{minipage}{\textwidth}
      \caption{\textbf{Weather super resolution.}  Description of the image. Description of the image. Description of the image. Description of the image. Description of the image. Description of the image. Description of the image.}
      \vspace{2mm}
      \includegraphics[width=\textwidth, height=8cm]{figure/weather_pred.png}
      % \experiments{Prediction of Weather SR} 
      \label{fig:weather_sr_pred}
    \end{minipage}
    \vspace{-5mm}

    % \begin{minipage}{\textwidth}
    %  \caption{\textbf{Spherical image super resolution.} Description of the image. Description of the image. Description of the image.}
     % \vspace{2mm}
     % \includegraphics[width=\textwidth, height=6.3cm]{section/sun360_pred.png}
     % \label{fig:sun360_sr_pred}
    % \end{minipage}
    

    
    % \begin{minipage}{\textwidth}
    %   \caption{\textbf{Test PSNR curve.} This is test PSNR curve for super resolution and regression task.}
    %   % \experiments{Error maps of CMB regression}
    %   \vspace{2mm}
      
    %   \includegraphics[width=\textwidth, height=4.2cm]{example-image-a}
    %   % \includegraphics[width=\textwidth]{figure/cmb_error_psnr.jpg}
    %   \label{fig:cmb_reg_error}
    % \end{minipage}%
\end{figure*}

==> figure/fig_wea_reg_psnr.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth, height=1in]{example-image-a}
    \vspace{-0.1in}
    \caption{\small \textbf{Test PSNR of regression in XX.}}
    \label{fig:weather_reg_psnr}
\end{figure}

==> figure/fig_wea_super_psnr.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figure/weather_psnr.png}
    \vspace{-0.1in}
    \caption{\small \textbf{Test PSNR of super-resolution in XX.}}
    \label{fig:weather_super_psnr}
\end{figure}

==> section/method.tex <==


\subsection{Problem Definition}
In this work, we investigate the encoding schemes of hybrid neural representation for two distinct types of data distribution: one centered on a pole and another that is uniformly distributed. These distributions exhibit varying characteristics by the latitudinal location. In addition, the spherical domain presents its own set of unique challenges: (1) same longitudinal line which is appeared as two separated lines on a equirectangular map (e.g., appearing at both 180° E and 180° W), (2) unitary pole position where the multiple contour lines passing through. To address these hurdles, we propose a promising hybrid representation encoding scheme that fully acknowledges the data distribution and unique characteristics inherent to the spherical domain.
\subsection{Method Description}

Our study involves a neural network that inputs spherical coordinates $\lbrace\mathbf{q}_i =(\theta_i,\phi_i)\lvert i\in\mathbb{N})\rbrace$ of data points and maps them to a target variable $\textbf{y}\in\mathbb{R}^d$. As illustrated in  \cref{fig:overview}, our method involves several key steps: (1) We adjust the distribution of learnable parameters to align with the actual data. Subsequently, our approach involves (2) the hierarchical construction of a multi-resolution grid of parameters and (3) the synthesis of these grid parameters to create multi-level latent codes for each input point. In this section, we will describe each process in detail.

\input{figure/fig_3_errormap}

\textbf{Data-driven parameter arrangement.} The essence of our approach lies in tailoring the arrangement of learnable parameters to match the actual data distribution. We examine two distinct data distributions: one non-uniformly centered around a pole and a uniform distribution across the sphere. For data with a pole-centered distribution, we represent this using an equirectangular projection map, a format often used for weather data~\cite{hersbach2018era5, rasp2020weatherbench}. In this case, we place the parameters at the corners of the equirectangular map.  Consequently, to manage the singularity at the poles, we utilizes a single parameter for both the North and South Poles respectively. Similarly, to address the spherical nature's periodicity, a unified parameter is required for the East-end ($180^\circ$E) and West-end ($180^\circ$W). For uniformly distributed data, we represent it using a HEALPix (Hierarchical Equal Area Isolatitude Pixelization) map, which is widely used for cosmological data~\cite{collaboration2015planck, abolfathi2018fourteenth, perez2018dark}. Unlike equirectangular map, HEALPix map pixel is uniformly spaced and covers equal areas, regardless of pixel location. Here, the grid parameters are positioned at the pixel's center. The choice of parameter location, whether at a corner or center of a pixel, is optional. The effect of parameter arrangement can be seen in the ~\cref{fig:case-error-map}. If the grid arrangement doesn't align with the actual data distribution, capturing the data distribution's signals in certain areas becomes challenging. For instance, if the grid parameters are uniformly arranged but the actual data is concentrated around the pole, the model struggles to detect signals near the pole, and the opposite is true for other distributions.

\textbf{Hierarchical parameter grid.} Our approach adopts a hierarchical parameter grid where the grid map's scale varies by level. This hierarchical approach allows to capture coarse to fine details while easily applicable for both equirectangular and HEALPix map. To be specific, for the equirectangular map, we begin at a base resolution $b$ and scales up the resolution by multiplying the upscale factor $\gamma$. Thus, at level $l$, the resolution of the map becomes $b\cdot \gamma^m$. The dimension of the grid map for each level becomes $H_l=$, $W_l=$. For the HEALPix map, its resolution is decided by $N_\text{side}$ parameter which indicates the divisions along the side of the coarsest resolution pixel. The coarsest resolution is defined as $N_\text{side}=2^0$ where total number of the pixel is 12. Consequently, each level $l$, the resolution is set by $N_\text{side}=2^l$ making the the total number of the pixel on the map $12\cdot N_\text{side}^2$. To sum up, our method encoding scheme is defined as : 
\begin{align*}
& \mathbf{Z}:=(Z_0,\ldots,Z_L) & \\
& Z_l :=(\mathbf{z}_i^l)\in\mathbb{R}^{n_l\times F},\quad \text{for } l\in[1,L] & \\
& \mathbf{z}_i^l\in\mathbb{R}^F,\quad \text{for } i\in[1,n_l] &
\end{align*}
where $n_l=H_l\times W_l$ for equirectangular grid and $n_l=12(N_{\text{side}}^l)^2$ for HEALPix grid.

\textbf{Parameter synthesis.} Once we've arranged the hierarchical grid parameters, we synthesize the input representation for each data point. For each query points we directly utilizes its coordinates to map onto a specific pixel in the parameter map and gather neighbor parameters which is close to the query points. To be specific,  for the equirectangular map we first normalizes and adjust these coordinates to fit with the bounds of an equirectangular grid. Then we scales the coordinates by its map resolution and obtain the four neighbor parameters which encloses the scaled coordinates. For the HEALPix map, we infer the four closest neighbor parameters by using a swift computational indexing method \textit{ang2pix}~\cite{gorski2005healpix}.
After we obtain the neighbor parameters, we calculate the distance between those neighbor parameters and query points and perform bilinear interpolation. To sum up, we can conclude the latent code for the query point as :
\begin{equation}
    \mathbf{z}_i=\bigoplus^L_{l=1}\text{Bi-Lerp}(\mathbf{q}_i,\mathcal{N}_l(\mathbf{q}_i))
\end{equation}

where $\mathbf{z}_i\in\mathbb{R}^{L\cdot F}$ is a latent code for query point $q_i$ and $\mathcal{N}_l(q_i)$ is a neighbor parameters of the $\mathbf{q_i}$ at level $l$. Finally the MLP takes the encoded parameter $\mathbf{z}\in\mathbb{R}^{N\times L\cdot F}$ and predicts the target variable $\mathbf{y}\in\mathbb{R}^d$ : 
\begin{equation}
    \mathbf{y} = f_\theta(\mathbf{z}),\quad\text{with }\mathbf{z}=\lbrace \mathbf{z}_i\lvert i\in\mathbb{N}\rbrace
\end{equation}

\textbf{Further Extension.} We can employ a hashing technique to reduce the size of parameter grid, similar to the approach used in neural graphic primitives~\cite{muller2022instant}. However, given that our method primarily addresses weather and CMB data, which are significantly larger and expand more extensively due to additional parameters like time and pressure, we opt to fully exploit the parameters at each grid level. Nevertheless, our approach could be made more adaptive and compact by aligning with the distribution of training samples, potentially implementing a optimized HEALPix arrangement, referred to as mHEALPix ~\cite{martinez2022multiresolution}, and adaptively refining the block grids ~\cite{martel2021acorn}. Exploring these enhancements will be part of our future research.

==> table/tab_ablation.tex <==
\begin{table}[h]
    \centering
    \captionof{table}{\textbf{Ablation study for algorithmic components of the equirectangular grid for XX task.} The evaluation metric is weighted PSNR and the best metric is highlighted in \textbf{bold}.}
    \label{tab:ablation}
    \vspace{0.1in}

    \resizebox{0.42\textwidth}{!}{
     \begin{tabular}{ccc}
        \toprule
        Pole singularity & Periodicity & Weighted PSNR \\
        %Pole singularity & Periodicity &   \\
        \midrule
        \xmark & \xmark  & 61.27 \\
        \cmark & \xmark &   61.30\\
        \xmark & \cmark &   61.25\\
        \cmark & \cmark &  \textbf{61.34} \\ 
        \bottomrule
      \end{tabular}
    }    
\end{table}


==> table/tab_cmb_reg.tex <==
% \begin{figure}[h]

%     \centering
%     % \caption{CMB denoising with $N_{\text{side}}$=$\lbrace512, 1024\rbrace$.}
%     \captionof{table}{\textbf{Results of cosmology data for regression.} The evaluation is based on PSNR and the best metric is highlighted in \textbf{bold}.}
%     \label{tab:cmb_reg}
%     \vspace{0.1in}
 
%           \resizebox{0.3\textwidth}{!}{
%      \begin{tabular}{lccc}
%         \toprule
%         & CMB \\
%         \midrule
%         ReLU+P.E. & 24.42 &  \\ 
%         SIREN &28.30 & \\ 
%         SHINR & 28.30 & \\ 
%         WIRE & 30.07 &  \\ 
%         FFN & 28.39 &  \\ 
%         % SMICA &  &   \\
%         \midrule
%         Ours & \textbf{38.72} & \\
%         \bottomrule
%       \end{tabular}}
% \end{figure}

==> table/tab_concept.tex <==
\centering
\begin{tabular}{lccc}
    \toprule
    Condition & i & ii & iii \\
    \midrule
    Freq (2D)  & \xmark & \xmark & \cmark  \\
    Freq (3D)  & \cmark & \cmark & \xmark  \\
    Hybrid (2D) & \xmark & \xmark & \cmark \\
    Hybrid (3D) & \cmark & \cmark & \xmark\\
    \midrule
    Ours & \cmark & \cmark & \cmark  \\
    \bottomrule
\end{tabular}

==> table/tab_main.tex <==
% % cite 빼면 별로 안 멋있어서 일단 넣어놨는데 빼도 됩니다,,
% \begin{table*}[t]
%     \caption{\textbf{Results on the real world datasets.} For the weather dataset including geopotential (Geo.) and temperature (Temp.) data, evaluation is based on weighted PSNR, while for the CMB dataset, it is assessed using standard PSNR. The best metric is highlighted in \textbf{bold}.}
%     \label{tab:main}
%     \vspace{0.1in}
%     \centering
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{lcccccccccccc}
%     \toprule
%     &\multicolumn{4}{c}{Super resolution (x2)} & \multicolumn{4}{c}{Super resolution (x4)} & \multicolumn{4}{c}{{Regression}} \\
%     \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
%     Method & Geo. & Temp. &SUN360 & CMB & Geo. & Temp. &SUN360 & CMB & Geo. & Temp. &SUN360 & CMB \\
%     \midrule
%     ReLU + P.E.\citep{mildenhall2021nerf} & 61.71 & 54.17 & 23.28 & 21.30 & 58.07 & 51.35 & 19.49 & 20.99 & 60.2 & 55.63 & - & 24.42 \\
%     SIREN \citep{sitzmann2020implicit} & 60.52 & 55.43 & 23.60 & 21.50 & 57.64 & 50.64 & 19.62 & 22.20 & 55.10 & 55.20 & - & 28.30 \\
%     SHINR \citep{esteves2022generalized}& 54.25 & 43.00 & 18.31 & 21.11 & 53.12 & 42.27 & 17.32 & 21.22 & 54.98 & 45.75 & - & 22.67 \\
%     WIRE \citep{saragadam2023wire} & 59.67 & 53.37 & 23.58 & 26.01 & 55.34 & 50.45 & 19.31 &25.78& 65.93 & 54.56 & - & 30.07 \\
%     FFN \citep{tancik2020fourier} & 62.04 & 56.15 & 24.32 & 23.98 & 56.62 & 51.97 & 19.73 & 23.53 & 61.15 & 57.14 & - & 28.39 \\
%     \midrule
%     \textbf{Ours} & \textbf{70.52} & \textbf{61.28} & \textbf{24.50} & \textbf{32.65}  & \textbf{61.17} & \textbf{53.93} & - & \textbf{30.37} & \textbf{66.17} & \textbf{63.45} & - & \textbf{38.72} \\
%     \bottomrule
%     \end{tabular}}
% \end{table*}
